TorchSparse: Efficient Point Cloud Inference Engine

Deep learning on point clouds has received increased attention thanks to its wide applications in AR/VR and autonomous driving. These applications require low latency and high accuracy to provide real-time user experience and ensure user safety. Unlike conventional dense workloads, the sparse and irregular nature of point clouds poses severe challenges to running sparse CNNs efficiently on the general-purpose hardware. Furthermore, existing sparse acceleration techniques for 2D images do not translate to 3D point clouds. In this paper, we introduce TorchSparse, a high-performance point cloud inference engine that accelerates the sparse convolution computation on GPUs. TorchSparse directly optimizes the two bottlenecks of sparse convolution: irregular computation and data movement. It applies adaptive matrix multiplication grouping to trade computation for better regularity, achieving 1.4-1.5x speedup for matrix multiplication. It also optimizes the data movement by adopting vectorized, quantized and fused locality-aware memory access, reducing the memory movement cost by 2.7x. Evaluated on seven representative models across three benchmark datasets, TorchSparse achieves 1.6x and 1.5x measured end-to-end speedup over the state-of-the-art MinkowskiEngine and SpConv, respectively.

==> figText/background/convs.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/background/compare_convs.pdf}
    \caption{\SparseConvolution on point clouds (b/c) is very different from conventional convolution (a): the activations always keep the sparsity pattern rather than dilating and the computation is guided by explicitly-computed \mappingpairs.}
    \label{fig:background:convs}
\end{figure*}

